Transportable Offline Reinforcement Learning in Presence of Unmeasured Confounding

Offline reinforcement learning seeks to learn decision policies from previously collected data, but deployment environments may differ from the domains in which the data were collected, and logged variables may omit confounders that affected both historical actions and outcomes. We study offline policy learning under the joint challenges of domain discrepancy and unmeasured confounding, where multiple heterogeneous source datasets provide complementary information about a target domain. We develop a causally adjusted transportability framework combining transportability theory with instrumental variables, negative controls, and proxies to identify target-domain causal quantities. For confounded contextual bandits, identification reduces to systems of bridge-function integral equations, enabling minimax estimation from finite samples. Confidence sets for the identified quantities are then used for pessimistic policy optimization, yielding CAT-CCB. We extend the framework to episodic confounded Markov decision processes, where complementary sources identify target reward and transition mechanisms under structural and completeness conditions. Under Gaussian dynamics and linear function approximation, this yields CAT-CMDP. We establish high-probability finite-sample suboptimality guarantees that quantify the effects of approximation, estimation, source-to-target shift, offline coverage, and sample size. For bounded finite-dimensional linear classes, the contextual-bandit guarantee recovers the standard $\widetilde{\mathcal O}(N^{-1/2})$ rate. Numerical experiments support the effectiveness of the framework for learning target-domain policies from heterogeneous confounded data. Together, the results provide a principled approach when no single source dataset suffices for causal identification and policy optimization.

==> chap1___old___.tex <==
\section{Introduction}
Offline reinforcement learning (RL) has emerged as a promising paradigm for deriving optimal decision-making policies from historical datasets, eliminating the need for costly or dangerous online interactions with the environment (\citealp{lange2012batch}; \citealp{levine2020offline}; \citealp{prudencio2023survey}). By leveraging large-scale static datasets, offline RL aims to democratize autonomous decision-making in fields ranging from healthcare (\citealp{raghu2018behaviour}; \citealp{gottesman2019guidelines}) to robotics (\citealp{kalashnikov2018scalable}; \citealp{fu2021benchmarks}). However, deploying RL systems in real‑world applications remains challenging, particularly when policies learned in experimental or simulated settings must be transferred to heterogeneous target environments (\citealp{levine2020offline, dulac2021challenges}). A central question we face in deploying these systems is: With datasets collected from heterogeneous sources, how can we recover the causal effect and learn an optimal strategy in the target system, in the presence of unmeasured confounding? (\citealp{bareinboim2016causal, kallus2018confounding, wang2021provably})

\paragraph{Key Challenges.} The transition from theoretical potential to practical deployment is currently hindered by three interconnected challenges: the distributional shift from source to target domain, unmeasured confounding, and insufficient data coverage.

In many practical scenarios, the environment where data is collected (the source domain) differs structurally from the environment where the policy must be applied (the target domain). This structural heterogeneity, known as domain discrepancy, arises not only from the inevitable oversimplification of experimental environments, but also from intrinsic differences between observational settings and real-world deployment contexts (\citealp{taylor2009transfer, levine2020offline, dulac2021challenges}). For instance, experimental designs valid in controlled settings may fail to capture the complex dynamics of real-world scenarios (\citealp{tobin2017domain, peng2018sim}). Furthermore, we frequently aim to leverage data from a well-studied domain to inform policy in a poorly studied one, where the underlying characteristics differ significantly (\citealp{Pearl_Bareinboim_2011, Lee_Correa_Bareinboim_2020}). A concrete instance of this is transferring policy insights from a developed urban region---characterized by advanced infrastructure and specific population demographics---to a rural region with limited infrastructure and different socioeconomic factors. Without accounting for these structural shifts, policies trained on source data may be ineffective or even harmful in the target environment (\citealp{schulam2017reliable, subbaswamy2019preventing}).

In complex systems, it is often expensive or impossible to record the state of every relevant factor, hence the source environments are often simplified approximations of the real world (\citealp{dulac2021challenges}). This oversimplification leads to unmeasured confounders-—inaccessible variables that influence both the actions taken by the logging policy and the rewards received (\citealp{pearl_2009, vdw13confounder}). For instance, in autonomous driving, unrecorded weather conditions or sensor noise might influence both the driver's braking patterns and the likelihood of an accident (\citealp{amodei2016concrete, michelmore2018evaluating}). Standard RL algorithms, which assume that all relevant state variables are observed (or at least that the unobserved ones do not confound the action-reward relationship), may mistakenly interpret these spurious correlations as causal mechanisms (\citealp{bareinboim2015bandits, lattimore2016causal}). Consequently, ``optimal'' policies learned from such data might be neutralized or biased by these hidden factors when deployed.

Finally, offline datasets are static and often suffer from insufficient coverage of the state-action space (\citealp{lange2012batch, levine2020offline, wang2020statistical}). Due to specific experimental designs, the collected data may only explore a small subset of possible behaviors, inducing a mismatch between behavioral policy and the optimal policy of interest (\citealp{fujimoto2019off, kumar2020conservative}). As a result, policy optimization in regions with scarce data can lead to unreliable extrapolation. This challenge necessitates the use of pessimism (\citealp{pmlr-v139-jin21e}), which optimizes against worst-case outcomes within a confidence set, improving robustness to statistical uncertainty.

These challenges are not merely theoretical; they are pervasive in high-stakes applications:
\begin{itemize}
\item In \emph{autonomous control and robotics}, policies are frequently trained in simulators or laboratory settings that omit rare disturbances, hardware imperfections, or complex human–environment interactions (\citealp{jakobi1995noise, peng2018sim}). These latent factors may influence both control actions and outcomes, inducing confounding in logged data, while deployment occurs under dynamics that differ from the training environment (\citealp{de2019causal}).

\item In \emph{operations research and resource allocation}, historical decisions—such as pricing, inventory management, or routing—are shaped by unobserved market conditions or managerial judgment (\citealp{besbes2012blind, athey2017state}). Datasets collected across regions or time periods therefore correspond to heterogeneous environments, and naive pooling can bias estimates of intervention effects.

\item In \emph{biomedicine}, clinical trials are conducted under strictly controlled protocols that may not account for the complex socioeconomic or genetic confounders present in the general patient population (\citealp{rothwell2005external, ackerman2021generalizing}). Learning an optimal treatment strategy for a new setting requires principled causal adjustment and transport across environments.

\item In \emph{social science and economics}, policy evaluation often relies on data from multiple jurisdictions or studies, where institutional differences and latent socioeconomic factors confound action–outcome relationships (\citealt{deaton2018understanding, vivalt2020much}). Transporting causal conclusions across settings is central to reliable policy design.
\end{itemize}

To address these challenges, we must move beyond purely statistical correlations and adopt a causal perspective. Our work employs the framework of Structural Causal Models (SCM) and Causal Directed Acyclic Graphs (DAGs) to explicitly model the data-generation processes (\citealp{pearl_2009}). Specifically, we employ the theory of transportability (\citealp{Pearl_Bareinboim_2011, Lee_Correa_Bareinboim_2020}), which provides a rigorous ``symbolic engine'' to determine if and how causal knowledge can be transferred across different environments. To handle the statistical uncertainty inherent in finite offline datasets, we integrate this causal framework with pessimism principle (\citealp{pmlr-v139-jin21e}) to construct lower confidence bounds on the expected reward to ensure robust policy learning.


\paragraph{Our Contribution.} In this paper, we propose a unified framework for transportable offline reinforcement learning that integrates causal identification and policy learning within a single principled approach. Our framework leverages multiple offline datasets collected from heterogeneous domains to recover causal effects and learn optimal decision policies in a target environment, even in the presence of structural heterogeneity and unmeasured confounding. In particular, our major contributions are four-fold:

\begin{itemize} 
\item\textit{Transportability across heterogeneity:} We establish a rigorous identification strategy that aggregates multiple datasets collected from heterogeneous source domains to recover the Conditional Average Treatment Effect (CATE) in a target domain. By integrating transportability theory with instrumental and proximal variable techniques, we derive integral equation systems (IES) that resolve identification even when unmeasured confounding and domain discrepancies prevent recovery from any single source domain.

\item\textit{Algorithm for causal estimation:} Building upon our identification results, we propose a minimax estimation procedure to solve the derived integral equation systems for bridge functions. We transform conditional moment equations into unconditional optimization problems, enabling the robust estimation of causal quantities (such as reward functions and transition kernels) from finite offline data.

\item\textit{Pessimistic policy optimization in dynamic settings:} We extend our framework from contextual bandits to confounded Markov Decision Processes (MDPs), proposing the Causal-Adjusted Transportable (CAT) algorithm. This approach constructs confidence sets for model parameters and employs a pessimistic principle to optimize the policy against the worst-case scenario, ensuring robustness against insufficient data coverage in the target domain.

\item\textit{Theoretical guarantees:} We provide comprehensive theoretical analysis characterizing the finite-sample performance of our algorithm. Specifically, we derive suboptimality bounds that explicitly account for the distribution shift between source and target domains, the complexity of function classes, and the strength of instrumental/proximal variables. \end{itemize}

By synthesizing tools from causal inference with pessimistic offline RL, this work provides a unified solution to the ``simulation-to-reality'' gap, enabling the learning of safe and effective policies in complex, partially observed environments.

\subsection{Related Works}
\paragraph{Structural causal models.} The application of structural equations and graph models traces back to some early work of econometrics (\citealp{wright1928tariff}; \citealp{strolz1960}; \citealp{goldberger1972structural}) and socilogy (\citealp{duncan1966}; \citealp{duane1974}), which traditionally assumes parametric or linear functional forms. To express the interrelation and control of variables in a economic system, a symbolic engine called \textit{do-calculus} (\citealp{judea1995}) for inference on causal directed acyclic graphs, which gives rise to a series of graph algorithms (\citealp{tian2002}; \citealp{shipster2006}; \citealp{Pearl_Bareinboim_2011}; \citealp{textor2012adjustment}). In further research, the structural causal models (\citealp{pearl_2009,Angrist2009,BPSM21}; \citealp{hm2023causal}) are developed, which form the basis for our discussion in this paper.

For adjustment of unmeasured confounding (\citealp{pearl_2009}; \citealp{vdw13confounder}), a large body of works in causal inference literature leverage side observations like instrumental variables (\citealp{angrist1996iv,nonparamivreg,Baiocchi2014,singh2020kernel}) and proxy variables (\citealp{miao2018identifying}; \citealp{miao2020confounding}; \citealp{tchetgen2020introduction,kallus2022causal,cui2023semiparametric}), which play a crucial role in identification of causal quantities associated with interventional distributions in structural causal models.


\paragraph{Transportability.} A central objective in causal inference is to extrapolate causal knowledge across domains, which is known as transportability (\citealp{Pearl_Bareinboim_2011}) or external validity (\citealp{pearl2022external}). Our framework builds on a series of works concentrating on the transportability of causal knowledge across heterogeneous domains (\citealp{Pearl_Bareinboim_2011}; \citealp{lee_ztrans}; \citealp{Bareinboim_Pearl_2013}; \citealp{pmlr-v31-bareinboim13a}; \citealp{bepj2014}; \citealp{Lee_Correa_Bareinboim_2020}; \citealp{softtrans2020}), which develop graphical and algebraic criteria for determining when causal quantities learned in one or more source domains can be validly transferred to a target domain. Among these works, the concepts of meta-transportability (\citealp{pmlr-v31-bareinboim13a}) and general transportability (\citealp{Lee_Correa_Bareinboim_2020}), focusing on the transportation from multiple source domains, are most relevant to this paper.

\paragraph{Offline reinforcement learning and Pessimism.} Offline RL aims to learn optimal policies from static historical datasets without further environment interaction (\citealp{levine2020offline}). Our work employs the pessimism principle (\citealp{liu2020provably,pmlr-v139-jin21e}; \citealp{xie2023bellmanconsistent}; \citealp{uehara2023pessimistic}) for offline reinforcement learning, which tackles with the challenge of distributional shift from observational to optimal policies (\citealp{wang2020statistical}; \citealp{levine2020offline}). Building on this foundation, numerous RL algorithms are designed to handle a variety of policy learning problems in presence of unmeasured confounding (\citealp{lu22prior}; \citealp{fu2022offline};  \citealp{chen2022instrumental}; \citealp{chen2023unified}; \citealp{lu2023pessimism, liao2021instrumental}). Recent work has also explored offline and transfer learning under heterogeneity and confounding (\citealp{mao2024stylized, gong2025provably}). Specifically, our work is closely related to \citealp{chen2023unified} and \citealp{liao2021instrumental}, as we adopt similar instrumental and proxy variables techniques from these studies.

\subsection{Preliminaries}
\paragraph{Structural causal models}(\citealp{pearl_2009}).  A structural causal model (SCM) is a quadruple $\mathcal{M}=(\mathbf{U},\mathbf{V},\mathcal{F},p)$, where
\begin{itemize}
\item $\mathbf{U}$ is a set of exogenous variables that are determined by factors outside the model. 
\item $\mathbf{V} = \lbrace V_1, \cdots , V_n\rbrace$ is a set of endogenous variables that are determined by factors in the model.
\item $\mathcal{F}$ is a set of functions $\lbrace f_1, \cdots, f_n\rbrace$ such that each $f_i$ is a mapping from  (the respective domains of) $U_i\cup Pa_i$ to $V_i,$ where $U_i\subseteq\mathbf{U}$ is some subset of $U$ whose elements are related to the variation of $V_i,$ $Pa_i\subseteq V\backslash V_i$ includes the parents of $V_i$ in the underlying causal DAG, and entire set of $F$ forms a mapping from $U$ to $V.$ In other words, $f_i$ assigns a value to the corresponding $V_i\in\mathbf{V},\ v_i\gets f(u_i,pa_i).$
\item $p$ is a probability distribution defined over the domain of $\mathbf{U}$, which creates variation in the endogenous variables $\mathbf{V}$.
\end{itemize}

Every SCM $\mathcal{M}$ gives rise to a directed acyclic graph (DAG) $\mathcal{G}(\mathcal{M}) = (\mathbf{V},\mathbf{E})$ (denoted as $\mathcal{G}$ for simplicity). Nodes in $\mathcal{G}$ correspond to endogenous variables in $\mathbf{V}$, and directed edges $\mathbf{E}$ emit from the set of parent nodes $Pa_i$ towards $V_i.$ This causal DAG specifies the causal mechanism according to which the data are generated.

Let $\mathcal{G}=(\mathbf{V},\mathbf{E})$ be a causal graph (DAG), and $\mathbf{A}$ be a subset of $\mathbf{V}$. Then we use $\mathcal{G}_{\overline{\mathbf{A}}}$ to denote the causal diagram induced by intervening on variables $\mathbf{A}$, i.e., the edges pointing to nodes in $\mathbf{A}$ are removed from $\mathcal{G}$. Similarly, let $\mathcal{G}_{\underline{\mathbf{A}}}$ denote the causal diagram resulting from removing edges that are emitted by nodes in $\mathbf{A}$.

\paragraph{Symbolic engine: do-calculus} (\citealp{judea1995}). We denote by $p(y|x,\mathrm{do}(z))$ the interventional distribution of $Y$ conditional $Z$ after intervening $Z=z$. Let $X, Y, Z$ and $W$ be arbitrary disjoint sets of nodes in $\mathcal{G}$. We use $p$ to stand for probability distribution. Do-calculus states the following three rules. To establish identifiability of a query $Q$, one needs to repeatedly apply the rules of do-calculus to $Q$ until the final expression no longer contains a do-operator.
\begin{itemize}
    \item Rule 1 (Insertion/deletion of observations).
  \begin{equation*}
      p(y\vert \mathrm{do}(x), z, w) = p(y\vert\mathrm{do}(x),w),\ \ \text{if}\ Y\perp Z\vert X,W\ \text{in}\ {\mathcal{G}_{\overline{X}}};
  \end{equation*}
  \item Rule 2 (Action/observation exchange).
  \begin{equation*}
  p(y\vert \mathrm{do}(x),\mathrm{do}(z), w) = p(y\vert\mathrm{do}(x),z, w),\ \ \text{if}\ Y\perp Z\vert X,W\ \text{in}\ {\mathcal{G}_{\overline{X},\underline{Z}}};\end{equation*}

  \item Rule 3 (Insertion/deletion of actions).
  \begin{equation*}
  p(y\vert \mathrm{do}(x),\mathrm{do}(z), w) = p(y\vert\mathrm{do}(x), w),\ \ \text{if}\ Y\perp Z\vert X,W\ \text{in}\ {\mathcal{G}_{\overline{X},\overline{Z(W)}}},\end{equation*}
  
where $Z(W)$ denotes the set of $Z$-nodes that are not ancestors of any $W$-nodes in $\mathcal{G}_{\overline{X}}$.
\end{itemize}

\paragraph{Selection diagram} (\citealp{Lee_Correa_Bareinboim_2020}). Suppose that both $\mathcal{M}^*$ and $\{\mathcal{M}^{(i)}\}_{i=1}^n$ conform to a causal graph $\mathcal{G}_0=(\mathbf{V},\mathbf{E})$. Then for any $i\in[n]$, we denote by $\Delta^{(i)}$ a set of variables such that for any $V\in\Delta^{(i)}$, there might exist a discrepancy: either the structural equations $f^{(i)}_V\neq f^*_V$ or $p^{(i)}(\mathbf{u}_V)\neq p^*(\mathbf{u}_V)$. Moreover, let $\mathbf{C}=\{C_V\,|\,V\in\bigcup_{i=1}^n\Delta^{(i)}\}$ be selection variables. Then $\mathcal{G}_0$ can be augmented. A selection diagram is defined as a graph $\mathcal{G}=(\mathbf{V}\cup\mathbf{C},\mathbf{E}\cup\{C_V\to V\}_{C_V\in \mathbf{C}})$.

We denote $\mathcal{M}^{(i)}$-specific variables by $\mathbf{C}^{(i)}=\{C_V\}_{V\in\Delta^{(i)}}$, and the remainder by $\mathbf{C}^{(-i)}=\mathbf{C}\backslash\mathbf{C}^{(i)}$. Then the range of a selection variable $C_V$ is $\{*\}\cup\{i|V\in\Delta^{(i)}\}$. Consequently, the selection diagram $\mathcal{G}$ can be viewed as a unifying SCM where the selection variables works like switches specifying the SCM of interest:
\begin{equation}
	p(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{x},\mathbf{C}^{(i)}=i,\mathbf{C}^{(-i)}=*) = p^{(i)}(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{x}).
\end{equation}

\paragraph{S-admissibility} (\citealp{Pearl_Bareinboim_2011}). A set of variables $\mathbf{Z}$ is said to be an S-admissible set between $\mathcal{M}^*$ and $\mathcal{M}^{(i)}$ with respect to the causal effect of $\mathbf{A}$ on $\mathbf{Y},$ if
\begin{equation*}
\left(\mathbf{C}^{(i)}\indep\mathbf{Y}|\mathbf{Z}\right)_{\mathcal{G}_{\overline{\mathbf{A}}}},
\end{equation*}
where $\mathcal{G}_{\overline{\mathbf{A}}}$ is induced by removing all arrows towards nodes in $\mathbf{A}$ from the selection diagram $\mathcal{G}$. Moreover, we have the direct transportability:
\begin{equation}
p^*(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{w}) = p^{(i)}(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{w}).\label{dteq}
\end{equation}
\begin{proof}
By equation (\ref{dteq}) and do-calculus rule 1, we have
\begin{align*}
	p^*(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{w}) 
	&= p(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{x},\mathbf{C}^{(i)}=*,\mathbf{C}^{(-i)}=*)\\
	&= p(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{x},\mathbf{C}^{(i)}=i,\mathbf{C}^{(-i)}=*)
	= p^{(i)}(\mathbf{y}|\mathrm{do}(\mathbf{a}),\mathbf{w}),
\end{align*}
which concludes the proof.
\end{proof}

\paragraph{Rademacher complexity and critical radius.} Suppose we have a function class $\mathcal{F}:\mathcal{X}\to\mathbb{R}$ that is uniformly bounded by $b$, i.e. $\forall f\in\mathcal{F},\Vert f\Vert_\infty \leq b$. The localized empirical Rademacher complexity of a function class $\mathcal{F}$ based on a sample $\{x_i\}_{i=1}^n$ is defined as
\begin{equation}
	\mathcal{R}(\delta;\mathcal{F},x_{1:n}) := \E\left[\sup_{f\in\mathcal{F}:\Vert f\Vert_{P_n}\leq\delta}\frac{1}{n}\sum_{i=1}^n\epsilon_if(x_i)\right],\label{radcomp}
\end{equation}
where $\{\epsilon_i\}_{i=1}^n$ are independent Rademacher variables, i.e. $\mathbb{P}(\epsilon_i=1) = \mathbb{P}(\epsilon_i=-1) = 1/2$, and $\Vert\cdot\Vert_{P_n}$ is the $L_2$ norm with respect to empirical distribution $P_n:=\frac{1}{n}\sum_{i=1}^n \delta_{x_i}$. The empirical critical radius of $\mathcal{F}$ on dataset $\{x_i\}_{i=1}^n$ is defined as the minimum positive solution to $\mathcal{R}(\delta;\mathcal{F},x_{1:n})\leq\delta^2/b$:
\begin{equation}
	\widehat{\delta}_n := \min\left\{\delta > 0:\mathcal{R}(\delta;\mathcal{F},x_{1:n})\leq\frac{\delta^2}{b}\right\}.\label{criticalradius}
\end{equation}
\paragraph{Notations.} We use capital letters like $X,A,Y$ to denote random variables, and use the corresponding calligraphic letters like $\mathcal{A},\mathcal{X},\mathcal{Y}$ to denote their range.  Suppose $\mathcal{A}$ is a measurable space, we let $\Delta(\mathcal{A})$ denote the family of probability distributions over $\mathcal{A}$. We write $X\indep Y$ if random variables $X$ and $Y$ are independent, and we write $X\indep Y\,|\,Z$ if they are conditionally independent given variable $Z$. For any $H\in\mathbb{N}$, we use $[H]$ to denote consecutive integers from $1$ to $H$, i.e. $[H] = \{1,2,\cdots,H\}$. We denote by $L^2(\mathcal{X},\mu)$ by the $L^2$-space (i.e. the square-integrable functions) defined on a measure space $(\mathcal{X},\mu)$, and we omit $\mu$ if there is no ambiguity. For any function $f$, we let $\mathcal{O}(f)$ denote the functions that increase as fast as $f$, i.e. there exists constants $C_1,C_2>0$ such that $C_1f\leq \mathcal{O}(f)\leq C_2f$. We let $\widetilde{O}(f)$ denote $\mathcal{O}(f\cdot\mathrm{poly}(\log f))$.

\subsection{Roadmap}
In \S\hyperref[sec:2]{2}, we discuss the impact of domain discrepancy in unconfounded contextual bandits and the possibility of leverage it with transportability, and we also formalize the problem setting in presence of unmeasured confounders. In \S\hyperref[sec:3]{3}, we discuss how to use transportability to identify causal quantities introduced in \S\hyperref[sec:2]{2} in some typical contextual bandits. In \S\hyperref[sec:4]{4}, we discuss the estimation of conditional moments, and propose our algorithm CAT-CCB to solve the offline policy learning problem in confounded contextual bandits. In \S\hyperref[sec:5]{5}, we expand the setting of domain discrepancy to Markov decision processes (MDPs) in presence of unobserved confounders, and discuss the causal identification in confounded MDPs using instrumental variables. In \S\hyperref[sec:6]{6}, we further propose our CAT-CMDP algorithm to solve the offline policy learning problem discussed in \S\hyperref[sec:5]{5} under Gaussian dynamics. Finally, in \S\hyperref[sec:7]{7}, we provide convergence analysis of our CAT algorithms proposed in \S\hyperref[sec:4]{4} and \S\hyperref[sec:6]{6} under regular conditions.

==> figs/chap8.tex <==
\section{Numerical Experiments}
\label{sec:experiments}
% =====================================================================
%  Experiments section for the CAT offline RL paper (discrete redesign).
%
%  Main-text figure files (place in figs/, which \graphicspath points to):
%     fig_identification_subopt.pdf   fig_rate.pdf
%     fig_cmdp_identification.pdf     fig_cmdp_pessimism.pdf
%  Appendix figure files:
%     fig_sensitivity.pdf  fig_calibration.pdf  fig_phase.pdf
%
%  Side-by-side panels use minipage, so this file does NOT depend on the
%  subfigure or subcaption packages.
% =====================================================================

We evaluate the framework on two deliberately transparent discrete structural causal models: the confounded contextual bandit (CCB-Neg) of Section~\ref{sec:3} and the confounded MDP of Section~\ref{sec:5}. Finite state and action spaces make the true bridge functions and the target causal quantities available in closed form, the empirical minimax loss exactly quadratic, the confidence set exactly an ellipsoid, and the policy class enumerable, so every reported number is measured against ground truth. Full model specifications, coefficients, and protocols are in Appendix~\ref{app:scm} (CCB-Neg) and Appendix~\ref{app:cmdp} (CMDP); the pessimism analysis, the bound-quantity sensitivity study, and the radius calibration are in Appendix~\ref{app:exp-pessimism}.

The main text reports the results that bear most directly on the central claims: that the multi-source construction recovers the target causal quantity while each ingredient is necessary (Sections~\ref{sec:exp-identification} and~\ref{sec:exp-cmdp-perf}), that the suboptimality scales with sample size as the theory suggests (Section~\ref{sec:exp-rate}), and that the sequential deconfounding keeps the suboptimality flat in the horizon while the baselines' confounding bias compounds (Section~\ref{sec:exp-cmdp-perf}).

\subsection{Confounded Contextual Bandits}\label{sec:exp-ccbneg}

\paragraph{Data-generating process.}
We use a discrete CCB-Neg model with $K = 6$ context strata $X$ and $M = 5$ actions $A$, a negative outcome $W$, an action instrument $Z_A \in \mathbb{R}^M$, a negative-outcome instrument $Z_W \in \mathbb{R}$, and an unobserved confounder $U$ that confounds $A$, $W$, and $Y$. The reward surface is cell-saturated and linear in $W$, $f^{(d)}(w,a,x) = \mu^{(d)}_x + b^{(d)}_x w + \tau^{(d)}_{x,a} + \lambda^{(d)}_a w$, and two source domains realize the complementary discrepancies of Assumption~\ref{assumption:3.1}: source~$1$ preserves the reward mechanism but shifts the $W$-mechanism and behavior policy ($\Delta^{(1)} = \{A,W\}$), while source~$2$ preserves the $W$-mechanism but shifts the reward mechanism and behavior policy ($\Delta^{(2)} = \{A,Y\}$). Neither source alone transports to the target. Their identified components combine through
\begin{equation}
\label{eq:exp-identification}
g^\star(a,x) = \mathbb{E}^{(2)}\!\bigl[\, h_1^\star(W,a,x) \mid X=x \,\bigr], \qquad h_1^\star = f^\star,
\end{equation}
where the reward bridge $h_1^\star$ is identified in source~$1$ through the instrumental moment restriction and the target $W$-law is supplied by source~$2$. Since $\mathbb{E}^{(2)}[W \mid X=x] = \omega^\star_x$ in closed form, the target causal mean $g^\star$ and the optimal policy $\pi^\star(x) = \arg\max_a g^\star(a,x)$ are known exactly. The instrument moment conditions condition on $(X, Z_A, Z_W)$ rather than on the realized action; conditioning on the realized cell would condition on $U$ through the action and reintroduce the selection bias. The cell-saturated bases make the minimax loss admit the closed form of Section~\ref{sec:4}, with Hessian $\widehat Q = \widehat J^\top \widehat\Omega^{-1} \widehat J$ and exact ellipsoid $\mathcal C_\theta(r) = \{\theta : \tfrac12 (\theta-\hat\theta)^\top \widehat Q (\theta-\hat\theta) \le r\}$; the full estimation procedure is in Appendix~\ref{app:ccb-neg-estimation}.

\paragraph{Methods.}
The \textsc{Full} method combines all three ingredients: multi-source identification, instrumental deconfounding, and the contrast-centered pessimistic policy of Appendix~\ref{app:exp-pessimism}. We compare it against one-ingredient ablations: \textsc{CAT, no pessimism} is the transported point estimate without the pessimistic correction; \textsc{Source1-Only} and \textsc{Source2-Only} apply the instrumental adjustment within a single source and so omit transport; \textsc{Transport-NoIV} performs the transport split but replaces the instrument test functions with cell indicators and so omits deconfounding; \textsc{Naive-Pool} regresses $Y$ on CATE cell indicators over the pooled sources with no causal adjustment. We report suboptimality $\mathrm{SubOpt} = v^{\pi^\star} - v^{\hat\pi}$, averaged over $60$ seeds with error bars of one standard error.

\subsubsection{Identification and the necessity of each component}
\label{sec:exp-identification}

We run the methods in the setting the theory targets: a harmful reward regime on the two hard contexts together with a partial-coverage hole there, and a coverage-stressed first source ($n_1 = n/8$), while varying the second-source size $n$. Figure~\ref{fig:identification} shows that \textsc{Full} attains the lowest suboptimality across the whole range, decreasing from $0.14$ to $0.095$, while every other method stays trapped near a bias floor between $0.18$ and $0.30$. The point estimate \textsc{CAT, no pessimism} is lured by the optimizer's curse into the poorly supported harmful actions and does not recover with sample size; the ablations each plateau on the floor set by the ingredient they omit. The separation between \textsc{Full} and \textsc{Transport-NoIV} reflects deconfounding, and the separation between \textsc{Full} and \textsc{Source1-Only} reflects transport. These results provide empirical evidence consistent with the identification result of~\eqref{eq:exp-identification}; the identification and consistency statements themselves are established by the theory.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.66\linewidth]{fig_identification_subopt.pdf}
  \caption{%
    Suboptimality against per-source sample size $n$ (log-log axes), in the harmful partial-coverage regime. The full method is lowest across the whole range; the point estimate and every ablation stay trapped on a bias floor set by the ingredient they omit. Curves show the mean over $60$ seeds and error bars show one standard error.}
  \label{fig:identification}
\end{figure}

\subsubsection{Finite-sample scaling}
\label{sec:exp-rate}

Theorem~\ref{thm:7.3} bounds the policy suboptimality, so we study the finite-sample scaling of the suboptimality itself. Because the rate characterizes the statistical estimation term rather than any residual coverage bias, this diagnostic is run in the benign, full-coverage regime, where the statistical term dominates. Figure~\ref{fig:rate} fits a power law to the suboptimality of the full method: its slope is steeper than the $n^{-1/2}$ reference, consistent with a statistically consistent estimator whose policy regret vanishes with sample size, while the deconfounding-free ablation flattens because its error is dominated by a bias floor rather than by sampling variance. We present this as an empirical scaling diagnostic and do not read it as a verification of the theorem.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.62\linewidth]{fig_rate.pdf}
  \caption{%
    Finite-sample scaling of the suboptimality on log-log axes, benign regime. Markers show the mean suboptimality at each $n$, solid lines the fitted power law with slope $\hat b$ in the legend, and the dotted line the $n^{-1/2}$ reference. The full method decays with sample size; the bias-dominated ablation flattens.}
  \label{fig:rate}
\end{figure}

\subsection{Confounded MDP}
\label{sec:exp-cmdp}

The sequential methods of Section~\ref{sec:5} raise two questions the bandit model cannot address: whether the transport-plus-deconfounding construction still identifies the target value once applied at every stage, and whether the confounding bias of the baselines compounds with the horizon. We repeat the identification analysis on a discrete confounded MDP, built to the same standard of auditability; the full specification is in Appendix~\ref{app:cmdp}.

\paragraph{Model and estimators.}
We use a finite confounded MDP with $|\mathcal{S}| = 4$ states, $|\mathcal{A}| = 4$ actions, and horizon $H = 5$. At each stage an unobserved confounder enters the behavior policy, the reward, and the transition, so a direct regression on the realized state-action pair is biased; a negative-outcome proxy $W$ and instruments play the same roles as in the bandit model. Two source domains realize the complementary discrepancies of Assumption~\ref{assumption:3.1}, with source~$1$ preserving the reward and transition mechanisms and source~$2$ preserving the proxy mechanism. The target reward means, transition kernel, and optimal value are computed in closed form by marginalizing over $(W, U)$. Following Algorithm~\ref{alg:1} for CMDPs, the reward and transition bridges are estimated in source~$1$ by the instrumental moment restriction at each stage and transported to the target proxy law supplied by source~$2$, then combined by backward induction; we call this estimator \textsc{CAT-CMDP (per step)}. Because the structural mechanisms are stationary across stages, a variant pools the moment equations over the $H$ stages when forming the bridge, which reduces the per-stage variance; we call it \textsc{CAT-CMDP (pooled)} and use it as the primary estimator, with the per-step estimator shown to confirm that the pooling only reduces variance and does not change the limit. The ablations are the sequential analogues of the bandit case.

\subsubsection{Identification and horizon dependence}
\label{sec:exp-cmdp-perf}

Figure~\ref{fig:cmdp-identification}(a) varies the per-source trajectory count $n$. Both CAT-CMDP estimators converge toward the exact optimum while each ablation settles onto a bias floor; the pooled estimator attains the lowest suboptimality throughout, and the per-step estimator (which matches Algorithm~\ref{alg:1} exactly) converges to the same neighborhood with higher variance, so the pooling is a pure variance reduction under the stationary mechanisms. The separations reproduce the bandit conclusions in the sequential setting: deconfounding separates CAT-CMDP from \textsc{Transport-NoIV}, and transport separates it from \textsc{Source1-Only}. Figure~\ref{fig:cmdp-identification}(b) fixes the sample size and varies the horizon $H$: the suboptimality of CAT-CMDP stays flat across $H \in \{2, \dots, 10\}$, whereas the confounding bias of the baselines compounds with the horizon, with \textsc{Naive-Pool} growing from $0.149$ at $H = 2$ to $0.924$ at $H = 10$. The sequential deconfounding therefore prevents the per-stage bias from accumulating, which is the central qualitative prediction for the MDP case. The partial-coverage behavior carries over as well: a contrast-centered pessimistic variant retains the reference-policy safety guarantee as coverage collapses (Appendix~\ref{app:exp-pessimism}, Figure~\ref{fig:cmdp-pessimism}).

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_cmdp_identification.pdf}
  \caption{%
    Confounded MDP. (a) Suboptimality against per-source trajectory count $n$ (log-log axes): both CAT-CMDP estimators converge while each ablation settles onto a bias floor; the pooled estimator is lowest and the per-step estimator (Algorithm~\ref{alg:1}) reaches the same neighborhood with higher variance. (b) Suboptimality against horizon $H$ at fixed sample size (log-scale $y$-axis): CAT-CMDP stays flat while the confounding bias of the baselines compounds. Curves show the mean over $40$ seeds and error bars show one standard error.}
  \label{fig:cmdp-identification}
\end{figure}

\subsection{Summary}
\label{sec:exp-summary}

The experiments instantiate the framework on the CCB-Neg and confounded MDP models and provide empirical evidence consistent with the theory. In both settings the full method recovers the target causal quantity and attains the lowest suboptimality, each one-ingredient ablation settles onto the bias floor set by the ingredient it omits (Figures~\ref{fig:identification} and~\ref{fig:cmdp-identification}), and the suboptimality scales with sample size as the statistical analysis suggests (Figure~\ref{fig:rate}). The sequential deconfounding keeps the suboptimality flat in the horizon while the baselines' confounding bias compounds. The pessimism analysis, the bound-quantity sensitivity study, and the radius calibration are developed in Appendix~\ref{app:exp-pessimism}; an empirical study of the mediator variant is left to future work.

